Snapshot Ensembles: Train 1, get M for free

Ensembles of neural networks are known to be much more robust and accurate than individual networks. However, training multiple deep networks for model averaging is computationally expensive. In this paper, we propose a method to obtain the seemingly contradictory goal of ensembling multiple neural networks at no additional training cost. We achieve this goal by training a single neural network, converging to several local minima along its optimization path and saving the model parameters. To obtain repeated rapid convergence, we leverage recent work on cyclic learning rate schedules. The resulting technique, which we refer to as Snapshot Ensembling, is simple, yet surprisingly effective. We show in a series of experiments that our approach is compatible with diverse network architectures and learning tasks. It consistently yields lower error rates than state-of-the-art single models at no additional training cost, and compares favorably with traditional network ensembles. On CIFAR-10 and CIFAR-100 our DenseNet Snapshot Ensembles obtain error rates of 3.4% and 17.4% respectively.

==> fastEnsemble - arXiv/abstract.tex <==
%!TEX root=main.tex
Ensembles of neural networks are known to be much more robust and accurate than individual networks. However, training multiple deep networks for model averaging is computationally expensive. In this paper, we propose a method to obtain the seemingly contradictory goal of \emph{ensembling multiple neural networks at no additional training cost}.
We achieve this goal by training a single neural network, converging to several local minima along its optimization path and saving the model parameters.  To obtain repeated rapid convergence, we leverage recent work on cyclic learning rate schedules.
The resulting technique, which we refer to as \emph{Snapshot Ensembling}, is simple, yet surprisingly effective.  We show in a series of experiments that our approach is compatible with diverse network architectures and learning tasks. It consistently yields  lower error rates than state-of-the-art single models at no additional training cost, and compares favorably with traditional network ensembles. On CIFAR-10 and CIFAR-100 our DenseNet \name{}s obtain error rates of $3.4\%$ and $17.4\%$ respectively.

%
%Our main observation is that we can perturb a model with large learning rate and quickly drive it to convergence at a different minimum with small learning rate. By using multiple, short training cycles, we can obtain a number of models without increasing computational overhead.
%We show different learning cycles can yield highly divergent models, with good precision. These models can then be effectively ensembled to achieve improved performance.


==> fastEnsemble - arXiv/analytic.tex <==
%!TEX root=main.tex
% \section{Discussion}
% Our method is compatible with other techniques (batch normalization, dropout etc.). 



==> fastEnsemble - arXiv/conclusion.tex <==
%!TEX root=main.tex
\section{Discussion}

We introduce Snapshot Ensembling, a simple method to obtain ensembles of neural networks without any additional training cost. 
Our method exploits the ability of SGD to converge to and escape from local minima as the learning rate is lowered, which allows the model to visit several weight assignments that lead to increasingly accurate predictions over the course of training. We harness this power with the cyclical learning rate schedule proposed by~\citet{loshchilov2016sgdr}, saving model snapshots at each point of convergence. We show in several experiments that all snapshots are accurate, yet produce different predictions from one another, and therefore are well suited for test-time ensembles.
Ensembles of these snapshots significantly improve the state-of-the-art on CIFAR-10, CIFAR-100 and SVHN.
Future work will explore combining Snapshot Ensembles with traditional ensembles. 
In particular, we will investigate how to balance growing an ensemble with new models (with random initializations) and refining existing models with further training cycles under a fixed training budget.

\section*{Acknowledgements}

We thank Ilya Loshchilov and Frank Hutter for their insightful comments on the cyclic cosine-shaped learning rate. The authors are supported in part by the, III-1618134, III-1526012, IIS-1149882 grants from the National Science Foundation, US Army Research Office W911NF-14-1-0477, and the Bill and Melinda Gates Foundation. 

% \para{Parallel \name{}s.}
% The short learning rate annealing cycles also provide a new way to improve traditional ensemble training. In particular, we can consider the short learning rate cycle as a new primitive for training rather than a long annealing process. Ensembles can be constructed either by training a single model for multiple cycles (\name{}) or by training multiple models (with different random initializations) for few cycles each. As an example, given a budget of $M=6$ short cycles, we can train $K=1$ model with $M=6$ cycles, or $K=2$ independent models with $M=3$ cycles each, etc. In theory, these cycles could be allocated dynamically, choosing to improve existing models or train new ones by greedily minimizing the validation error. The optimal trade-off between number of cycles $M$ and number of parallel initializations $K$ is still open research. 


==> fastEnsemble - arXiv/experiments.tex <==
%!TEX root=main.tex
\section{Experiments}
\label{sec:results}



We demonstrate the effectiveness of Snapshot Ensembles on several benchmark datasets, comparing with competitive baselines. We run all experiments with Torch 7~\citep{torch}\footnote{Code to reproduce results is available at \url{https://github.com/gaohuang/SnapshotEnsemble}}.


\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
& {\bf Method} &  & {\bf C10} & {\bf C100} & \bf{SVHN} & \bf{Tiny ImageNet}\\
%&& & {\bf scheduling}  & \\
\midrule
\multirow{5}{*}{{ ResNet-110}}  &  Single model &  & 5.52 &  28.02 & 1.96 & 46.50\\
%&  Dropout (0.2) &  &   &    &  &  \\
&  NoCycle Snapshot Ensemble &  &  5.49 &  26.97 & 1.78 & 43.69 \\
%&  SingleCycle Ensembles (STD LR) & & 7.35 & 26.30  & 1.81 & 45.50 \\
&  SingleCycle Ensembles & & 6.66 & 24.54  & 1.74 & 42.60\\
&  Snapshot Ensemble ($\alpha_0=0.1$) &  &  \textcolor{blue}{5.73} &  \textcolor{blue}{25.55} & \textcolor{blue}{\bf 1.63}  & \textcolor{blue}{40.54} \\
&  Snapshot Ensemble ($\alpha_0=0.2$) &  &  \textcolor{blue}{{\bf 5.32}} &  \textcolor{blue}{{\bf 24.19}} & \textcolor{blue}{1.66} & \textcolor{blue}{\bf 39.40} \\
\midrule
\multirow{6}{*}{{ Wide-ResNet-32}}  &  Single model &  &  5.43  &  23.55  & 1.90 & 39.63 \\
&  Dropout &  & 4.68  &  22.82  & 1.81  & 36.58 \\
&  NoCycle Snapshot Ensemble &  &  5.18 &  22.81 & 1.81 & 38.64\\
%&  SingleCycle Ensembles (STD LR) && 5.86 & 21.97  & 1.68  & 36.88\\
&  SingleCycle Ensembles && 5.95 & 21.38  & 1.65  & 35.53\\
&  Snapshot Ensemble ($\alpha_0=0.1$) &  &  \textcolor{blue}{{\bf 4.41}} &  \textcolor{blue}{{\bf 21.26}}  & \textcolor{blue}{1.64} & \textcolor{blue}{35.45}\\
&  Snapshot Ensemble ($\alpha_0=0.2$) &  &  \textcolor{blue}{4.73} &  \textcolor{blue}{21.56} &  \textcolor{blue}{{\bf 1.51}} & \textcolor{blue}{{\bf 32.90}}\\
\midrule
\multirow{6}{*}{{ DenseNet-40}} &  Single model &   &  5.24$^*$ &  24.42$^*$ & 1.77 & 39.09 \\
&  Dropout &  &  6.08 &  25.79 & 1.79$^*$ & 39.68 \\
&  NoCycle Snapshot Ensemble &  &  5.20 &  24.63  & 1.80 & 38.51 \\
%&  SingleCycle Ensembles (STD LR) && 5.55 & 22.85 & 2.03 & 40.43 \\
&  SingleCycle Ensembles & & 5.43 & 22.51  & 1.87 & 38.00  \\
%&  Ensemble 3 independent smaller models\footnotemark &  &  5.31 &  25.39 & & \\
%&  Ensemble 3 pre-mature models (100 epochs)   &  5.17 &  22.83 & & \\
&  Snapshot Ensemble ($\alpha_0=0.1$) &  &  \textcolor{blue}{4.99} &  \textcolor{blue}{23.34}  & \textcolor{blue}{{\bf 1.64}}  & \textcolor{blue}{37.25} \\
&  Snapshot Ensemble ($\alpha_0=0.2$) &  &  \textcolor{blue}{{\bf 4.84}} &  \textcolor{blue}{{\bf 21.93}}  & \textcolor{blue}{1.73}& \textcolor{blue}{{\bf 36.61}} \\
%&  Snapshot Ensemble (ours) &  (10-30-5-5) &  5.20 &  22.30  & & \\
%&  Snapshot Ensemble (ours) &  (0-40-5-5) &  4.96 &  22.91  & & \\
%&  Snapshot Ensemble (ours) &  100$\times$ 3 &  cosine annealing &  5.34 &  22.80  & & \\
\midrule
\multirow{6}{*}{{ DenseNet-100}}  &  Single model &  &  3.74$^*$ &  19.25$^*$ & - & - \\
&  Dropout &  &  3.65 &  18.77 & - & - \\
&  NoCycle Snapshot Ensemble & &  3.80  &  19.30  & - & -\\
%&  SingleCycle Ensembles (STD LR) &&  4.39 & 18.70 & - & - \\
&  SingleCycle Ensembles  & & 4.52 & 18.38  &  &  \\

&  Snapshot Ensemble ($\alpha_0=0.1$) &   &   \textcolor{blue}{{3.57}} &   \textcolor{blue}{{18.12}}  & \textcolor{blue}{-} & \textcolor{blue}{-} \\
&  Snapshot Ensemble ($\alpha_0=0.2$) &   &   \textcolor{blue}{{\bf 3.44}} &   \textcolor{blue}{{\bf 17.41}}  & \textcolor{blue}{-} & \textcolor{blue}{-} \\
%&  Snapshot Ensemble (ours) &  100 $\times$ 3&  cosine annealing &  {\bf 3.57} &  {\bf 18.12}  & & \\
\bottomrule
\end{tabular}
\caption[]{\small Error rates ($\%$) on CIFAR-10 and CIFAR-100 datasets. All methods in the same group are trained for the same number of iterations. Results of our method are colored in \textcolor{blue}{blue}, and the best result for each network/dataset pair are {\bf bolded}. $^*$ indicates numbers which we take directly from \cite{huang2016densely}.}
\label{table:results}
\end{table*}


%
%
%\begin{table*}[t]
%\centering
%\small
%\begin{tabular}{lcccccc}
%\toprule
%& {\bf Method} & & {\bf lr } & {\bf C10} & {\bf C100} & \bf{SVHN}\\
%&& & {\bf scheduling} \\
%\midrule
%\multirow{3}[3]{*}{{ ResNet-110}}  &  Single model & &  standard &  6.27$^*$ &  27.66$^*$ &\\
%&  NoCycle Snapshot Ensemble & &  standard &  {\bf 6.16} &  27.09 &\\
%&  Snapshot ensemble & &  cosine annealing (0.1) &  6.40 &  {\bf 26.37} & \\
%\midrule
% &  Single model & &  standard &  5.43$^*$  &  23.55$^*$  &\\
%%&  Stochastic Depth~\citep{stochastic} & &  standard &  5.23 &  24.58 & \\
%\multirow{1}[3]{*}{{ Wide-ResNet-32}}  &  NoCycle Snapshot Ensemble & &  standard &  5.18 &  22.81 &\\
%&  Snapshot ensemble & &  cosine annealing (0.1) &  {\bf 4.41} &  {\bf 21.26}  &\\
%&  Snapshot ensemble & &  cosine annealing (0.2) &  4.73 &  21.56 & \\
%\midrule
%&  Single model &  &  standard &  5.24 &  24.42 &\\
%&  Dropout (0.2) & &  standard &  6.08 &  25.79 & \\
%\multirow{1}[3]{*}{{ DenseNet-40}} &  NoCycle Snapshot Ensemble & &  standard &  5.20 &  24.63  &\\
%%&  Ensemble 3 independent smaller models\footnotemark & &  standard &  5.31 &  25.39 &\\
%%&  Ensemble 3 pre-mature models (100 epochs)  &  standard &  5.17 &  22.83 &\\
%&  Snapshot ensemble & &  cosine annealing (0.1) &  4.99 &  23.34  &\\
%&  Snapshot ensemble & &  cosine annealing (0.2) &  {\bf 4.84} &  {\bf 21.93}  &\\
%%&  Snapshot ensemble (ours) & &  standard (10-30-5-5) &  5.20 &  22.30  &\\
%%&  Snapshot ensemble (ours) & &  standard (0-40-5-5) &  4.96 &  22.91  &\\
%%&  Snapshot ensemble (ours) &  100$\times$ 3 &  cosine annealing &  5.34 &  22.80  &\\
%\midrule
% &  Single model & &  standard &  3.74 &  19.25 &\\
%&  Dropout (0.2) & &  standard &  - &  - &\\
%\multirow{1}[3]{*}{{ DenseNet-100}} &  NoCycle Snapshot Ensemble &&  standard &  3.80  &  19.30  &\\
%&  Snapshot ensemble &  &  cosine annealing (0.1) &  {3.57} &  {18.12}  &\\
%&  Snapshot ensemble &  &  cosine annealing (0.2) &  {\bf 3.44} &  {\bf 17.41}  &\\
%%&  Snapshot ensemble (ours) &  100 $\times$ 3&  cosine annealing &  {\bf 3.57} &  {\bf 18.12}  &\\
%\bottomrule
%\end{tabular}
%\caption[]{\small Error rates ($\%$) on CIFAR-10 and CIFAR-100 datasets. All methods in the same group use the same amount of training time and cost. Results that surpasses all competing methods are bold. $^*$ indicates results reproduced by ourselves.}
%\label{table:results}
%\end{table*}



\subsection{Datasets}
\para{CIFAR.}
The two CIFAR datasets \citep{cifar} consist of colored natural images sized at 32$\times$32 pixels. CIFAR-10 (C10) and CIFAR-100 (C100) images are drawn from 10 and 100 classes, respectively.
For each dataset, there are 50,000 training images and 10,000 images reserved for testing. %, and we hold out 5,000 training images as the validation set.
We use a standard data augmentation scheme \citep{netinnet, fitnet, dsn, allcnn, highway, stochastic, fractalnet}, in which the images are zero-padded with 4 pixels on each side, randomly cropped to produce 32$\times$32 images, and horizontally mirrored with probability $0.5$.

%We denote this augmentation scheme by a ``+'' mark at the end of the dataset name (\emph{e.g.}, C10+). %For data preprocessing, we normalize the data using the channel means and standard deviations. We evaluate our algorithm on all four datasets: C10, C100, C10+, C100+. For the final run we use all 50,000 training images and report the final test error at the end of training.

\para{SVHN.}
The Street View House Numbers (SVHN) dataset~\citep{svhn} contains $32\times32$ colored digit images from Google Street View, with one class for each digit. There are 73,257 images in the training set and 26,032 images in the test set. Following common practice~\citep{sermanet2012convolutional, maxout, huang2016densely}, we withhold 6,000 training images for validation, and train on the remaining images without data augmentation.
%All the images are normalized to the scale $[0,1]$ for preprocessing.

\para{Tiny ImageNet.}
The Tiny ImageNet dataset\footnote{\url{https://tiny-imagenet.herokuapp.com}} consists of a subset of ImageNet images~\citep{deng2009imagenet}. There are 200 classes, each of which has 500 training images and 50 validation images. Each image is resized to $64\times64$ and augmented with random crops, horizontal mirroring, and RGB intensity scaling~\citep{alexnet}.

\para{ImageNet.} The ILSVRC 2012 classification dataset \citep{deng2009imagenet} consists of 1000 images classes, with a total of 1.2 million training images and 50,000 validation images. We adopt the same data augmentation scheme as in \citep{he2016deep,huang2016densely} and apply a $224\times 224$ center crop to images at test time.

 \begin{figure*}[t]
\centerline{
                \includegraphics[width=0.49\linewidth]{figures/l100_k24_ensemble_singlerow-crop.pdf}
            \includegraphics[width=0.49\linewidth]{figures/l100_k24_ensemble_singlerow_02-crop.pdf}}
% }        \begin{subfigure}[b]{\linewidth}
%             \centering
%             \vspace{0.2em}
%         \end{subfigure}
%         \begin{subfigure}[b]{\linewidth}
%             \centering
%         \end{subfigure}
%         \caption[]
        \caption{\small DenseNet-100 Snapshot Ensemble performance on CIFAR-10 and CIFAR-100 with restart learning rate $\alpha_0=0.1$ (left two) and $\alpha_0=0.2$ (right two). Each ensemble is trained with $M\!=\!6$ annealing cycles (50 epochs per each).}
        \label{fig:free-ensemble-barplot}
        \vspace{-1em}
    \end{figure*}

\subsection{Training Setting}

\para{Architectures.} We test several state-of-the-art architectures, including residual networks ({\bf ResNet})~\citep{he2016deep}, {\bf Wide ResNet}~\citep{wide} and {\bf DenseNet}~\citep{huang2016densely}.
For ResNet, we use the original 110-layer network introduced by \cite{he2016deep}. Wide-ResNet is a 32-layer ResNet with 4 times as many convolutional features per layer as a standard ResNet. For DenseNet, our large model follows the same setup as ~\citep{huang2016densely}, with depth $L=100$ and growth rate $k=24$. In addition, we also evaluate our method on a small DenseNet, with depth $L=40$ and $k=12$. To adapt all these networks to Tiny ImageNet, we add a stride of $2$ to the first layer of the models, which downsamples the images to $32\times32$. For ImageNet, we test the 50-layer ResNet proposed in \citep{he2016deep}.
We use a mini batch size of 64.\footnote{Exceptions: ResNet-110 and Wide-ResNet are trained with batch size 128 on Tiny ImageNet. The ImageNet model is trained with batch size 256.}

\para{Baselines.} Snapshot Ensembles incur the training cost of a single model; therefore, we compare with baselines that require the same amount of training. First, we compare against a {\bf Single Model} trained with a standard learning rate schedule, dropping the learning rate from $0.1$ to $0.01$ halfway through training, and then to $0.001$ when training is at $75\%$.
Additionally, to compare against implicit ensembling methods, we test against a single model trained with {\bf Dropout}. This baseline uses the same learning rate as above, and drops nodes during training with a probability of $0.2$.

We then test the {\bf Snapshot Ensemble} algorithm trained with the cyclic cosine learning rate as described in \eqref{eq:lr-cosine}. We test models with the max learning rate $\alpha_0$ set to $0.1$ and $0.2$.
In both cases, we divide the training process into learning rate cycles. Model snapshots are taken after each learning rate cycle.
Additionally, we train a Snapshot Ensemble with a non-cyclic learning rate schedule. This {\bf NoCycle Snapshot Ensemble}, which uses the same schedule as the Single Model and Dropout baselines, is meant to highlight the impact of cyclic learning rates for our method.
To accurately compare with the cyclic Snapshot Ensembles, we take the same number of snapshots equally spaced throughout the training process.
Finally, we compare against {\bf SingleCycle Ensembles}, a Snapshot Ensemble variant in which the network is re-initialized at the beginning of every cosine learning rate cycle, rather than using the parameters from the previous optimization cycle.
This baseline essentially creates a traditional ensemble, yet each network only has $1/M$ of the typical training time.
%The model is trained using a standard learning rate cycle of $\left\lceil T/M\right\rceil$ iterations, after which the model is re-initialized.
This variant is meant to highlight the tradeoff between model diversity and model convergence. Though SingleCycle Ensembles should in theory explore more of the parameter space, the models do not benefit from the optimization of previous cycles.
% For each of the variants, we test the ensemble by feeding samples through each model snapshot and averaging the softmax outputs.

\para{Training Budget.} On CIFAR datasets, the training budget is $B=300$ epochs for DenseNet-40 and DenseNet-100, and $B=200$ for ResNet and Wide ResNet models. Snapshot variants are trained with $M=6$ cycles of $B/M=50$ epochs for DenseNets, and $M=5$ cycles of $B/M=40$ epochs for ResNets/Wide ResNets.
SVHN models are trained with a budget of $B=40$ epochs ($5$ cycles of $8$ epochs). For Tiny ImageNet, we use a training budget of $B=150$ ($6$ cycles of $25$ epochs). Finally, ImageNet is trained with a budget of $B=90$ epochs, and we trained 2 Snapshot variants: one with $M=2$ cycles and one with $M=3$.

\begin{wraptable}{r}{0.5\textwidth}
\centering
\small
% \vspace{-1em}
\begin{tabular}{cc}
\toprule
Method & {\bf Val. Error (\%)} \\
\midrule
Single model & 24.01 \\
Snapshot Ensemble ($M = 2$) & 23.33 \\
Snapshot Ensemble ($M = 3$) & 23.96 \\
\bottomrule
\end{tabular}
\caption[]{\small Top-1 error rates ($\%$) on ImageNet validation set using ResNet-50 with varying number of cycles.}
\label{table:imagenet}
 \end{wraptable}

\subsection{Snapshot Ensemble results}

\para{Accuracy.} The main results are summarized in Table~\ref{table:results}. In most cases, Snapshot ensembles achieve lower error than any of the baseline methods. Most notably, Snapshot Ensembles yield an error rate of $17.41\%$ on CIFAR-100 using large DenseNets, far outperforming the record of $19.25\%$ under the same training cost and architecture~\citep{huang2016densely}. Our method has the most success on CIFAR-100 and Tiny ImageNet, which is likely due to the complexity of these datasets. The softmax outputs for these datasets are high dimensional due to the large number of classes, making it unlikely that any two models make the same predictions. Snapshot Ensembling is also capable of improving the competitive baselines for CIFAR-10 and SVHN as well, reducing error by $1\%$ and $0.4\%$ respectively with the Wide ResNet architecture.

The NoCycle Snapshot Ensemble generally has little effect on performance, and in some instances even \emph{increases} the test error.
This highlights the need for a cyclic learning rate for useful ensembling.
The SingleCycle Ensemble has similarly mixed performance.
In some cases, e.g., DenseNet-40 on CIFAR-100, the SingleCycle Ensemble is competitive with Snapshot Ensembles. However, as the model size increases to 100 layers, it does not perform as well. This is because it is difficult to train a large model from scratch in only a few epochs.
These results demonstrate that Snapshot Ensembles tend to work best when utilizing information from previous cycles.
Effectively, Snapshot Ensembles strike a balance between model diversity and optimization.

%Additionally, the optimal learning rate of Snapshot Ensembling appears to be dependent on dataset and architecture. We propose a more thorough investigation of these hyperparameters as future work.

Table \ref{table:imagenet} shows Snapshot Ensemble results on ImageNet.
The Snapshot Ensemble with $M=2$ achieves $23.33 \%$ validation error, outperforming the single model baseline with $24.01\%$ validation error. It appears that 2 cycles is the optimal choice for the ImageNet dataset.
Provided with the limited total training budget $B=90$ epochs, we hypothesize that allocating fewer than $B/2 = 45$ epochs per training cycle is insufficient for the model to converge on such a large dataset.


\begin{wraptable}{r}{0.25\textwidth}
\centering
\small
% \vspace{-1em}
\begin{tabular}{cc}
\toprule
{$M$} & {\bf Test Error (\%)} \\
\midrule
2 & 22.92 \\
4 & 22.07 \\
6 & 21.93 \\
8 & 21.89 \\
10 & 22.16\\
\bottomrule
\end{tabular}
\caption[]{\small Error rates of a DenseNet-40 Snapshot Ensemble on CIFAR-100, varying $M$---the number of models (cycles) used in the ensemble.}
\label{table:vary-block}
 \end{wraptable}


\para{Ensemble Size.} In some applications, it may be beneficial to vary the size of the ensemble \emph{dynamically} at test time depending on available resources. Figure~\ref{fig:free-ensemble-barplot} displays the performance of DenseNet-40 on the CIFAR-100 dataset as the effective ensemble size, $m$, is varied. Each ensemble consists of snapshots from later cycles, as these snapshots have received the most training and therefore have likely converged to better minima. Although ensembling more models generally gives better performance, we observe significant drops in error when the second and third models are added to the ensemble. In most cases, an ensemble of two models outperforms the baseline model.

% \begin{wraptable}{r}{0.6\textwidth}
%  \centering
%  \small
%  \begin{tabular}{cccc}
%  \toprule
%    {\bf Configurations $K\times M$} & {\bf lr scheduling} & {\bf C10} & {\bf C100}\\
%   \midrule
%    \cite{huang2016densely} &   standard & 5.24 & 24.42\\
%  Snapshot Ensemble (1$\times$6) & cyclical (0.1) & 4.99 & 23.34 \\
%  Snapshot Ensemble (2$\times$3) & cyclical (0.1) & 5.34 & 22.80 \\
%  Snapshot Ensemble (3$\times$2) & cyclical (0.1) & 5.34 & 22.80 \\
%  Snapshot Ensemble (6$\times$1) & cyclical (0.1) & 5.43 & 22.51 \\
%   \midrule
%  Snapshot Ensemble (1$\times$6) & cyclical (0.2) & 4.84 & 21.93 \\
%  Snapshot Ensemble (2$\times$3) & cyclical (0.2) & 4.93 & 21.38 \\
%  Snapshot Ensemble (3$\times$2) & cyclical (0.2) & 4.89 & 21.04 \\
%  Snapshot Ensemble (6$\times$1) & cyclical (0.2) & 4.86 & 21.57 \\
%   \bottomrule
%   \end{tabular}
%  \caption[]{\small Error rates ($\%$) on CIFAR-10 and CIFAR-100 datasets using DenseNet-40, with a budget of training 6 cycles. Each annealing cycle is trained for 50 epochs.}
%  \label{table:results-multirow}
%  %\end{wraptable}
% \end{wraptable}


\para{Restart Learning Rate.} The effect of the restart learning rate can be observed in Figure~\ref{fig:free-ensemble-barplot}.
The left two plots show performance when using a restart learning rate of $\alpha_0=0.1$ at the beginning of each cycle, and the right two plots show $\alpha_0=0.2$.
In most cases, ensembles with the larger restart learning rate perform better, presumably because the strong perturbation in between cycles increases the diversity of local minima.


\para{Varying Number of Cycles.} Given a fixed training budget, there is a trade-off between the number of learning rate cycles and their length. Therefore, we investigate how the number of cycles $M$ affects the ensemble performance, given a fixed training budget. We train a 40-layer DenseNet on the CIFAR-100 dataset with an initial learning rate of $\alpha_0=0.2$. We fix the total training budget $B=300$ epochs, and vary the value of $M\in\{2,4,6,8,10\}$. As shown in Table~\ref{table:vary-block}, our method is relatively robust with respect to different values of $M$. At the extremes, $M=2$ and $M=10$, we find a slight degradation in performance, as the cycles are either too few or too short. In practice, we find that setting $M$ to be $4\sim8$ works reasonably well.

\para{Varying Training Budget.}
The left and middle panels of Figure~\ref{fig:true-ensemble-and-vary-budget} show the performance of Snapshot Ensembles and SingleCycle Ensembles as a function of training budget (where the number of cycles is fixed at $M=6$). We train a 40-layer DenseNet on CIFAR-10 and CIFAR-100, with an initial learning rate of $\alpha_0$ = 0.1, varying the total number of training epochs from 60 to 300. We observe that both Snapshot Ensembles and SingleCycle Ensembles become more accurate as training budget increases. However, we note that as training budget decreases, Snapshot Ensembles still yield competitive results, while the performance of the SingleCycle Ensembles degrades rapidly. These results highlight the improvements that Snapshot Ensembles obtain when the budget is low. If the budget is high, then the SingleCycle baseline approaches true ensembles and outperforms Snapshot ensembles eventually. 

% \begin{table*}[htbp]
% \centering
% \small
% \begin{tabular}{cccccc}
% \toprule
% {number of cycles $M$} & {\bf 2} & {\bf 4} & {\bf 6} & {\bf 8} & {\bf 10}\\
% \midrule
% Snapshot Ensemble (cosine annealing 0.2) & 22.92 & 22.07 & 21.93 & 21.89 & 22.16\\
% \bottomrule
% \end{tabular}
% \caption[]{\small Error rates ($\%$) on CIFAR-100 using DenseNet-40 with varying number of cycles.}
% \label{table:vary-block}
% \end{table*}
% \para{Parallel Snapshot Ensembles.}
%  We also study the effectiveness of Snapshot Ensembles when parallel resources are available during training. Given the total training budget of $B=300$ epochs, we train in parallel $K=\{1,2,3,6\}$ models, each with $M=\{6,3,2,1\}$ cycles of 50-epoch cosine annealing. Table~\ref{table:results-multirow} shows the results of different parallel configurations. By exploiting the parallel snapshot ensemble training, we find the performance can be further improved on dataset containing highly diverse classes such as CIFAR-100.

%\begin{wrapfigure}{r}{0.4\textwidth}
%    \centering
%    \includegraphics[width=0.4\textwidth]{figures/l40_k12_true_ensemble-crop.pdf}
%    \caption{\small Performance comparison of Snapshot Ensembles with true ensembles.}
%    \label{fig:true-ensemble}
%\end{wrapfigure}
%
%
% \begin{wrapfigure}{r}{0.4\textwidth}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figures/l40_k12_vary_budget_ensemble.pdf}
%    \caption{\small Snapshot Ensembles under different training budget.}
%    \label{fig:vary-budget}
%\end{wrapfigure}

 \begin{figure*}[t]
        \centerline{
        \includegraphics[width=0.33\textwidth]{figures/l40_k12_vary_budget_ensemble-crop.pdf}
        \includegraphics[width=0.33\textwidth]{figures/l40_k12_vary_budget_ensemble_c100-crop.pdf}
        \includegraphics[width=0.33\textwidth]{figures/l40_k12_true_ensemble-crop.pdf}
        }
        \caption[]
        {\small Snapshot Ensembles under different training budgets on {\bf (Left)} CIFAR-10 and {\bf (Middle)} CIFAR-100.
        {\bf Right:} Comparison of Snapshot Ensembles with true ensembles.
        }
        \label{fig:true-ensemble-and-vary-budget}
        \vspace{-1em}
    \end{figure*}


\para{Comparison with True Ensembles.} We compare Snapshot Ensembles with the traditional ensembling method. The right panel of Figure~\ref{fig:true-ensemble-and-vary-budget} shows the test error rates of DenseNet-40 on CIFAR-100. The true ensemble method averages models that are trained with 300 full epochs, each with different weight initializations. Given the same number of models at test time, the error rate of the true ensemble can be seen as a lower bound of our method. Our method achieves performance that is comparable with ensembling of 2 independent models, but with the training cost of one model.


%\begin{wraptable}{r}

% CIFAR-100: 16.87%

% Baseline small models:
%4.36 and 21.24%

% TODO
% Ensemble of 3 independent 300 epochs (small models on cifar 10 and CIFAR-100 will be done soon)
% Start running two more large models (CIFAR-10 and CIFAR-100)


% \footnotetext{The depth $L=22$ and growth rate $k=12$ for a smaller model are chosen so that the training time of each individual model is $1/3$ of the small DenseNet. This makes the total training time of three independent smaller models comparable to others.}




% \subsection{Fast ensemble results}
% CIFAR-10 CIFAR-100: Small DenseNets
%
%\begin{table*}[htbp]
%\centering
%\small
%\begin{tabular}{lccccc}
%\toprule
%& {\bf row(s) $\times$ block(s)} && {\bf lr scheduling} & {\bf C10} & {\bf C100}\\
%\midrule
%& \cite{huang2016densely} &  & standard & 5.24 & 24.42\\
%& Snapshot Ensemble (1$\times$6) && cosine annealing (0.1) & 4.99 & 23.34 \\
%& Snapshot Ensemble (2$\times$3) && cosine annealing (0.1) & 5.23 & 22.54 \\
%& Snapshot Ensemble (3$\times$2) && cosine annealing (0.1) & 5.34 & 22.80 \\
%& Snapshot Ensemble (6$\times$1) && cosine annealing (0.1) & 5.43 & 22.51 \\
%\midrule
%& Snapshot Ensemble (1$\times$6) && cosine annealing (0.2) & 4.84 & 21.93 \\
%& Snapshot Ensemble (2$\times$3) && cosine annealing (0.2) & 4.93 & 21.38 \\
%& Snapshot Ensemble (3$\times$2) && cosine annealing (0.2) & 4.89 & 21.04 \\
%& Snapshot Ensemble (6$\times$1) && cosine annealing (0.2) & 4.86 & 21.57 \\
%\bottomrule
%\end{tabular}
%\caption[]{\small Error rates ($\%$) on CIFAR-10 and CIFAR-100 datasets using DenseNet-40. Each annealing cycle (block) is trained for 50 epochs.}
%\label{table:results-multirow}
%\end{table*}



\subsection{Diversity of model ensembles}

% initially
% starting at model 4, in the same local minimum.
% interpolating 5 and 6 cause a decrease in the test error, possibly due to that
\para{Parameter Space.} We hypothesize that the cyclic learning rate schedule creates snapshots which are not only accurate but also diverse with respect to model predictions. We qualitatively measure this diversity by visualizing the local minima that models converge to.
To do so, we linearly interpolate snapshot models, as described by~\cite{goodfellow2014qualitatively}.
Let $J \left(\theta\right)$ be the test error of a model using parameters $\theta$.
Given $\theta_1$ and $\theta_2$ --- the parameters from models 1 and 2 respectively --- we can compute the loss for a convex combination of model parameters: $J \left( \lambda \left( \theta_1 \right) + \left(1 - \lambda \right) \left( \theta_2 \right) \right)$,
where $\lambda$ is a mixing coefficient. Setting $\lambda$ to 1 results in a parameters that are entirely $\theta_1$ while setting $\lambda$ to 0 gives the parameters $\theta_2$. By sweeping the values of $\lambda$,
we can examine a linear slice of the parameter space. Two models that  converge to a similar minimum will have smooth parameter interpolations, whereas models that converge to different minima will likely have a non-convex interpolation, with a spike in error when $\lambda$  is between 0 and 1.

 \begin{figure*}[t]
        \centerline{\includegraphics[width=0.5\textwidth]{figures/parametric_cosine-crop.pdf}
        \includegraphics[width=0.5\textwidth]{figures/parametric_standard-crop.pdf}
        }
        % \begin{subfigure}[b]{\linewidth}
        %     \centering
        %     \includegraphics[width=\linewidth]{figures/l40_k12_interpolation_firstrow-crop.pdf}
        %     \vspace{0.2em}
        % \end{subfigure}
        % \begin{subfigure}[b]{\linewidth}
        %     \centering
        %     \includegraphics[width=\linewidth]{figures/l40_k12_interpolation_baseline-crop.pdf}
        % \end{subfigure}
        \caption[]
        {\small Interpolations in parameter space between the final model (sixth snapshot) and all intermediate snapshots. $\lambda=0$ represents an intermediate snapshot model, while $\lambda=1$ represents the final model.
        {\bf Left:} A Snapshot Ensemble, with cosine annealing cycles ($\alpha_0=0.2$ every $B/M=50$ epochs).
        {\bf Right:} A NoCycle Snapshot Ensemble, (two learning rate drops, snapshots every $50$ epochs).
        }
        \label{fig:parametric-plots}
        \vspace{-1em}
    \end{figure*}

\autoref{fig:parametric-plots} displays interpolations between the final model of DenseNet-40 (sixth snapshot) and all intermediate snapshots. The left two plots show Snapshot Ensemble models trained with a cyclic learning rate, while the right two plots show NoCycle Snapshot models.
$\lambda=0$ represents a model which is entirely snapshot parameters, while $\lambda=1$ represents a model which is entirely the parameters of the final model.
From this figure, it is clear that there are differences between cyclic and non-cyclic learning rate schedules.
Firstly, all of the cyclic snapshots achieve roughly the same error as the final cyclical model, as the error is similar for $\lambda=0$ and $\lambda=1$.
Additionally, it appears that most snapshots do not lie in the same minimum as the final model. Thus the snapshots are likely to misclassify different samples.
Conversely, the first three snapshots achieve much higher error than the final model. This can be observed by the sharp minima around $\lambda=1$, which suggests that mixing in any amount of the snapshot parameters will worsen performance. While the final two snapshots achieve low error, the figures suggests that they lie in the same minimum as the final model, and therefore likely add limited diversity to the ensemble.

% We denote by $w^{i}$ the model parameters obtained after $i$-th training cycle. In our case, $i=1,2,..,6$ since the entire training is divided into 6 chunks. For any two models parameterized by $w^{(i)}$ and $w^{(j)}$, a linearly interpolated model can be denoted by $\alpha w^{(i)} + (1-\alpha) w^{(j)}$. In Figure~\ref{fig:parametric-plots}, we plot the classification error for the linearly interpolated model, for each pair of $w^{(i)} (i\ne 6)$ and the last model $w^{(6)}$, with $\alpha$ varying from 0 to 2. The plot shows the model diversity between $w^{(i)} (i\ne 6)$ and $w^{(6)}$ progressively increases as $i$ decreases.

% % \begin{figure*}[t]
% %         \centering
% %         \begin{subfigure}[b]{\linewidth}
% %             \centering
% %             \includegraphics[width=0.9\linewidth]{figures/l40_k12_interpolation_baseline-crop.pdf}
% %             \vspace{0.2em}
% %         \end{subfigure}
% %         \begin{subfigure}[b]{\linewidth}
% %             \centering
% %             \includegraphics[width=0.9\linewidth]{figures/l100_k24_interpolation_baseline-crop.pdf}
% %         \end{subfigure}
% %         \caption[]
% %         {Parametric plots.}
% %         \label{fig:parametric-plots-baseline}
% %         \vspace{-1em}
% %     \end{figure*}



% In contrast, we also show in Figure~\ref{fig:parametric-plots-baseline} the parametric plots for baseline approach of ensembling intermediate models using standard learning rate scheduling. We interpolate the final single model at epoch 300 with all five previous intermediate models at every interval of 50 epochs. There are two salient observations can be drawn from this. First, interpolating models at epoch 250 and 300 result in an almost flattened curve (in red). The trend is similarly observable for the model at epoch 200 (in yellowgreen), when $\alpha\in[0,1]$. This implies that the 4th, 5th and last models converge to solutions with low model diversity across, hence making it undesirable for the purpose of model ensembling. On the other hand, early models at epoch 50, 100 and 150 are far less close to convergence, resulting in the interpolation with the last model (almost fully converged) suffer from a sharp performance degradation.


 \begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/l100_k24_corr-crop.pdf}
    \caption{\small Pairwise correlation of softmax outputs between any two snapshots for DenseNet-100. {\bf Left:} A Snapshot Ensemble, with cosine annealing cycles (restart with $\alpha_0=0.2$ every 50 epochs). {\bf Right:} A NoCycle Snapshot Ensemble, (two learning rate drops, snapshots every 50 epochs).}
    \label{fig:correlation}
\end{wrapfigure}
\para{Activation space.} To further explore the diversity of models, we compute the pairwise correlation of softmax outputs for every pair of snapshots. \autoref{fig:correlation} displays the average correlation for both cyclic snapshots and non-cyclical snapshots. Firstly, there are large correlations between the last 3 snapshots of the non-cyclic training schedule (right). These snapshots are taken after dropping the learning rate, suggesting that each snapshot has converged to the same minimum. Though there is more diversity amongst the earlier snapshots, these snapshots have much higher error rates and are therefore not ideal for ensembling. Conversely, there is less correlation between all cyclic snapshots (left). Because all snapshots have similar accuracy (as can be seen in \autoref{fig:parametric-plots}), these differences in predictions can be exploited to create effective ensembles.
% As expected, correlations are strongest between consecutive snapshots.



==> fastEnsemble - arXiv/intro.tex <==
%!TEX root=main.tex
\section{Introduction}


%% trying new spin
Stochastic Gradient Descent (SGD)~\citep{bottou2010large} and its accelerated variants~\citep{kingma2014adam,duchi2011adaptive} have become the de-facto approaches for optimizing deep neural networks. The popularity of SGD can be attributed to its ability to avoid and even escape spurious saddle-points and local minima~\citep{dauphin2014identifying}.
Although avoiding these spurious solutions is generally considered positive,
in this paper we argue that these local minima contain useful information that may in fact improve model performance.
% there may in fact be some value to these local minima and that simply leaving them on the way-side may be outright wasteful.
%In particular, the sets of errors made at these local minima are disjoint from the errors made by the final model, and therefore can be exploited for improved accuracy.

Although deep networks typically never converge to a global minimum, there is a notion of ``good'' and ``bad'' local minima with respect to generalization.  \citet{keskar2016large} argue that local minima with
flat basins tend to generalize better.
% Intuitively this may because these change less if, hypothetically, the training data were swapped for testing data.
%
SGD tends to avoid sharper local minima because gradients are computed from small mini-batches and are therefore inexact~\citep{keskar2016large}. If the learning-rate is sufficiently large, the intrinsic random motion across gradient steps prevents the optimizer from reaching any of the sharp basins along its optimization path. However, if the learning rate is small, the model tends to converge into the closest local minimum. These two very different behaviors of SGD are typically exploited in different phases of optimization~\citep{he2016deep}. Initially the learning rate is kept high to move into the general vicinity of a flat local minimum. Once this search has reached a stage in which no further progress is made, the learning rate is dropped (once or twice), triggering a descent, and ultimately convergence, to the final local minimum.

It is well established~\citep{kawaguchi2016deep} that the number of possible local minima grows exponentially with the number of parameters---of which modern neural networks can have millions. It is therefore not surprising that two identical architectures optimized with different initializations or minibatch orderings will converge to different solutions.  Although different local minima often have very similar error rates, the corresponding neural networks tend to make different mistakes. This diversity can be exploited through ensembling, in which multiple neural networks are trained  from different initializations  and then combined  with majority voting or averaging~\citep{caruana2004ensemble}. Ensembling  often leads to drastic reductions  in error rates. In fact, most high profile competitions, e.g. Imagenet~\citep{deng2009imagenet} or Kaggle\footnote{\url{www.kaggle.com}}, are won by ensembles of deep learning architectures.

Despite its obvious advantages, the use of ensembling for deep networks is not nearly as wide-spread as it is for other algorithms.
% For example decision trees are most commonly used in the form of Random Forests or Boosted ensembles~\citep{breiman2001random,friedman2001greedy}.
One likely reason for this lack of adaptation may be the cost of learning multiple neural networks.
% Whereas  decision trees are cheap and require mere seconds to construct,
Training deep networks can last for weeks, even on high performance hardware with GPU acceleration.
As the training cost for ensembles increases linearly, ensembles can quickly becomes uneconomical for most researchers without access to industrial scale computational resources.
% Although the training of deep net ensembles can be trivially parallelized, few have access to sufficient GPU servers that can be deployed in parallel for long durations. \gp{How's this?}


% n% It is known that neural networks contain numerous ``good'' local minima~\citep{dauphin2014identifying}.
% Due to random initialization and shuffled minibatches, it is improbable that any two models converge to the same minimum, and therefore models will likely have disjoint sets of errors.
% This property can be exploited by ensembling several models, which reduces overall variance as a result of averaging differing predictions~\citep{Goodfellow-et-al-2016-Book}.
% However, training deep networks is computationally expensive and can last for days or even weeks even on high performance hardware with GPU acceleration.
% %Training ensembles of them increases the cost linearly and quickly becomes prohibitive for most researchers without access to industrial scale computational resources.
% Although the training of deep net ensembles can be trivially parallelized, few have access to sufficient GPU servers that can be deployed in parallel for long durations. \gp{How's this?}


\begin{figure*}[t!]
\vspace{-2ex}
  \centerline{
  \includegraphics[width=0.45\textwidth]{figures/sgd_path.pdf}
    \includegraphics[width=0.45\textwidth]{figures/sgd_restart_path.pdf}
  }
%   \begin{subfigure}[t]{0.4\textwidth}
%     \centering

%   \end{subfigure}%
%   ~
%   \begin{subfigure}[t]{0.4\textwidth}
%   \vspace{-2ex}
% \centerline{
%   \end{subfigure}
  \caption{\small{\bf Left:} Illustration of SGD optimization with a typical learning rate schedule. The model converges to a minimum at the end of training. {\bf Right:} Illustration of Snapshot Ensembling. The model undergoes several learning rate annealing cycles, converging to and escaping from multiple local minima. We take a snapshot at each minimum for test-time ensembling.}
  \label{fig:paths}
\end{figure*}

In this paper we focus on the seemingly-contradictory goal of learning an ensemble of multiple neural networks \emph{without incurring any additional training costs}.
We achieve this goal with a training method that is simple and straight-forward to implement. 
Our approach leverages the non-convex nature of neural networks and the ability of SGD to converge to and escape from local minima on demand.  Instead of training $M$ neural networks independently from scratch, we let SGD converge $M$ times to local minima along its optimization path.
Each time the model converges, we save the weights and add the corresponding network to our ensemble. We then restart the optimization with a large learning rate to escape the current local minimum. More specifically, we adopt the cycling procedure suggested by~\cite{loshchilov2016sgdr}, in which the learning rate is abruptly raised and then quickly lowered to follow a cosine function.
Because our final ensemble consists of snapshots of the optimization path, we refer to our approach as \emph{Snapshot Ensembling}. \autoref{fig:paths} presents a high-level overview of this method.

In contrast to traditional ensembles, the training time for the entire ensemble is identical to the time required to train a \emph{single} traditional model.  During testing time, one can  evaluate and average the last (and therefore most accurate) $m$ out of $M$ models. Our approach is naturally compatible with other methods to improve the accuracy, such as data augmentation,  stochastic depth~\citep{stochastic}, or  batch normalization~\citep{batch-norm}.  In fact, \name{}s  can even be ensembled, if for example parallel resources are available during training.  In this case, an ensemble of $K$ \name{}s  yields $K\times M$  models at $K$ times the training cost.

We evaluate the efficacy of \name{}s on three state-of-the-art deep learning architectures for object recognition: ResNet~\citep{he2016identity}, Wide-ResNet~\citep{wide}, and DenseNet~\citep{huang2016densely}.  We show across four different data sets that Snapshot Ensembles almost always reduce error without increasing training costs. For example, on CIFAR-10 and CIFAR-100, \name{}s obtains error rates of $3.44\%$ and $17.41\%$ respectively.



==> fastEnsemble - arXiv/introOLD.tex <==
Averaging classifiers is an effective method to reduce model variance by approximating the expected classifier. Ensemble methods~\citep{breiman2001random,caruana2004ensemble,hansen1990neural,krogh1995neural,zhou2002ensembling} leverage this fact to obtain improved generalization performance~\cite{koren2009bellkor}. 
For example, the Random Forests~\cite{breiman2001random}  algorithm elevates the modest CART~\cite{breiman1984classification} algorithm to one of the most competitive classifiers within machine learning. 
Here, slightly modified CART trees are bagged~\cite{breiman2001random}, where each tree is trained on a different subset of the data (drawn uniformly with replacement) and splits are randomized. The additional randomization of the decision trees leads to high variance classifiers. This is advantageous as the ensemble size can be very large (in practice often exceeding 10,000 CART trees) due to the extremely efficient ID3 algorithm~\cite{quinlan1986induction}. The large number of classifiers ensures that even in the presence of high variance the ensemble average approaches the expected model (which would have zero model variance).  

In the wake of deep learning, ensembling is just as important as it has ever been. Nowadays most high profile competitions (e.g. Imagenet~\cite{deng2009imagenet} or Kaggle\footnote{\url{www.kaggle.com}}) are won by ensembles of deep learning architectures. As neural networks are often initialized with random weights, there appears to be a sufficient amount of natural variation that allows all networks to be trained on the entire data set. 

Training deep networks is computationally expensive and can last for days or even weeks even on high performance hardware with GPU acceleration. Training ensembles of them increases the cost linearly and quickly becomes prohibitive for most researchers without access to industrial scale computational resources. Although the training of deep net ensembles can be trivially parallelized, few have access to sufficient GPU servers that can be deployed in parallel for long durations. As a result, ensembles of deep nets are typically small---averaging only a hand-full of classifiers. Consequently, the ensemble average still has high variance and does not approach the expected model. 

% The ensemble method is very effective for neural networks. In most cases, neural network ensembles yield significantly better generalization performance than a single network.
% The recent winners of the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) \citep{imagenet} have all used multiple networks for their final predictions \citep{szegedy2015going,smallfilter,resnet}.
% Researchers have found that independently trained neural networks tend to make different mistakes on test data, and thus averaging the softmax scores or using a majority voting scheme can greatly reduce the chance of a wrong prediction. The diversity amongst models is a product of random initialization and training with stochastic gradient descent (SGD), coupled with the high degree of nonlinearity in neural networks \gp{Should this mention non-convexity?}. Due to its simpleness and effectiveness, the ensemble method is widely used in deep learning applications.

% Although neural networks ensembles have been widely studied and utilized \citep{hansen1990neural,krogh1995neural}, most existing works focuses on improving the generalization performance, with little concern about the cost of training ensembles. This may be explained by the fact that, until recently, the sizes of both datasets and models were relatively small, making it affordable to train tens or even hundreds of networks for model averaging. However, the situation is rapidly changing. Many datasets now contain millions of samples, and researchers must train very deep networks to achieve good performance on these large scale datasets. Even with the modern GPUs, a deep network may take days or weeks to train. Under limited resources, it becomes important to address the large cost of training neural network ensembles. 

One useful feature of SGD is that SGD does not get caught in local minima that it happens upon during the training process.
In fact, SGD can even escape the attraction of a local minimum.
Somehow cite Bengio.
Therefore, rather than preventing a model from visiting local minima, we allow the model to visit many local minima over the course of optimization, knowing that we can escape it again.
We take a model snapshot when we converge to a local minimum, and then perturb the model to let it escape that local minimum. Therefore, we end up with several models that have converged to various minima, which give us enough variety to converge to several different models.

% There are several methods which can lower this cost to a certain extent. 
% For example, one can use shorter networks for model averaging, or train each network for fewer iterations.
% While these methods reduce training time, both may sacrifice accuracy on a sufficiently challenging dataset.
% Even with careful hyperparameter selection, such an ensemble might 
% not outperform the simple baseline: training a single network under the same amount of cost.
% Alternatively, one could train a single deep network, but ensemble intermediate models at different iterations of training.
% This method does not introduce any additional training
% beyond training a single model, yet the accuracy gain is often insignificant as there is little diversity amongst the different
% training iterations.


%Although neural networks ensembles have been widely studied and applied in machine learning \citep{hansen1990neural,krogh1995neural}, most of existing works focus on improving the generalization performance, while few of them address the cost of training ensembles. This may be explained by the fact that one decade ago both the size of datasets and models were relatively small, and it was affordable to train tens or even hundreds of networks for model averaging. But the situation is changing rapidly. On one hand, many of the datasets we have now contain millions of samples; On the other hand, researchers have to train very deep networks to achieve good performances on these large scale datasets.
%
%Even with the modern GPUs, a deep network may take days or weeks to train. Under limited resources, it becomes important to address the problem of high training cost of neural network ensembles. Several recent works focus on reducing the test time cost of ensembles, by transferring or distilling the ``knowledge" of cumbersome ensembles into smaller networks \citep{bucilu¨£2006model,hinton2015distilling}.
%

% In recent years, researchers have developed effective techniques which create ``implicit'' ensembles from single networks \citep{dropout,wan2013regularization,stochastic,singh2016swapout,krueger2016zoneout}. For example, the Dropout \citep{dropout} method randomly drops nodes in the hidden layers during each mini-batch of training. This can be viewed as training exponential number of networks with heavy parameter sharing. At test time, these models are averaged to make the final prediction. The recently proposed stochastic depth network \citep{stochastic} and Swapout \citep{singh2016swapout} algorithm create similar implicit ensembles at test time. \gp{Maybe worth mentioning the ``Resnets are ensembles\ldots'' paper?}

In this paper, we introduce a simple idea to obtain a cheep yet effective neural network ensembles under a limited training budget.
Our method produces multiple neural networks that achieve a remarkable balance between diversity and accuracy, yet only requires the \emph{same cost training a single network}. We draw inspiration from the recent finding of \cite{loshchilov2016sgdr} and \cite{leslie2016cyclical} that cyclical learning rates give significant improvement over commonly used learning rate scheduling. Cyclical learning rates split the training process into multiple blocks, each of which has a full learning rate annealing cycle. In each block, large learning rates perturbs a well converged model and small learning rates quickly drive the model towards convergence at a new minimum. Consequently, each block (or learning rate cycle) provides a candidate model for ensembling. This disturbance at the beginning of each block produces intermediate models with substantial diversity, and are therefore far more effective for ensembling than intermediate models from a conventional learning rate schedule. 

The proposed method has several remarkable advantages: 1) it is possible to retrieve models with good performance early in the training process, as noted by \citet{loshchilov2016sgdr}; 2) it always gives a complete single model at the end of training, and one can further improve its performance by simply ensembling more models provided test time budget allows;
%, making it useful for test time cost sensitive learning; 
3) the method is general and is compatible with many other effective tools in deep learning, such as Bagging, Boosting, Dropout, Swapout, Stochastic depth and the Dense-sparse-dense training flow. In fact, our method can be even more effective when combined with some of these other techniques.

We show on several popular benchmark datasets that our method yields state-of-the-art performance with the ResNet~\citep{identity-mappings} and DenseNet~\citep{huang2016densely} architecture under the same amount of training cost as in previous works. We also introduce how to further improve model diversity and reduce cost at training time.

%Tested on ResNet and DenseNet. Also introduces how to reducing test time computation.









==> fastEnsemble - arXiv/macros.tex <==
% METHOD NAME
\newcommand{\methodname}{cheap ensemble}
\newcommand{\methodnamecap}{Cheap Ensemble}
\newcommand{\methodnameshort}{}
\newcommand{\methodnameshorts}{}

% Gradients Equations
\newcommand{\feati}{x_i}
%\newcommand{\concatfeati}{x_i}
\newcommand{\clsfeati}{y_i}
\newcommand{\featk}{x_k}
\newcommand{\clsfeatk}{y_k}
\newcommand{\loss}{L}
\newcommand{\featL}{x_L}
\newcommand{\clsfeat}{y}
% Inputs and outputs
\newcommand{\anyxs}{\ensuremath{\mathbf{x}}}
\newcommand{\anyys}{\ensuremath{\mathbf{y}}}

\newcommand{\bx}{\ensuremath{\mathbf{x}}}

\newcommand{\sourcexs}{\ensuremath{\mathbf{x^\mathcal{S}}}}
\newcommand{\sourceys}{\ensuremath{\mathbf{y^\mathcal{S}}}}

\newcommand{\targetxs}{\ensuremath{\mathbf{x^\mathcal{T}}}}
\newcommand{\targetys}{\ensuremath{\mathbf{y^\mathcal{T}}}}
\newcommand{\pseudotargetys}{\ensuremath{\mathbf{\hat{y}^\mathcal{T}}}}

% Classifier
\newcommand{\class}{\ensuremath{\eta}}
\newcommand{\classsource}{\ensuremath{f_s}}
\newcommand{\classtarget}{\ensuremath{f_t}}

% Distributions
\newcommand{\xspace}{\ensuremath{X}}
\newcommand{\yspace}{\ensuremath{Y}}
\newcommand{\sourced}{\ensuremath{\mathcal{S}}}
\newcommand{\targetd}{\ensuremath{\mathcal{T}}}
\newcommand{\source}{\ensuremath{p}}
\newcommand{\target}{\ensuremath{q}}
\newcommand{\layeroutsource}[1]{\ensuremath{p_{H#1}}}
\newcommand{\layerouttarget}[1]{\ensuremath{q_{H#1}}}

% Network
\newcommand{\layer}{\ensuremath{\mathcal{L}}}
\newcommand{\perturb}{\ensuremath{\Delta \mathbf{h}}}
\newcommand{\layerout}{\ensuremath{\mathbf{h}}}
\newcommand{\layerfun}{\ensuremath{f}}
\newcommand{\resfun}{\ensuremath{\mathbf{c}}}
\newcommand{\sumfun}{\ensuremath{\mathbf{\bar{h}}}}

% Objective function
\newcommand{\lossmmd}{\ensuremath{\ell^{mmd}}}
\newcommand{\lossclsmmd}{\ensuremath{\ell^{mmd\prime}}}
\newcommand{\lossce}{\ensuremath{\ell^{ce}}}
\newcommand{\lossreg}{\ensuremath{\ell^{reg}}}

% Probability
\newcommand{\ev}{\ensuremath{\mathbb{E}}}
\newcommand{\mmd}{\ensuremath{\text{MMD}}}
\newcommand{\funcclass}{\ensuremath{\mathcal{F}}}

% Shorthands
\newcommand{\tup}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\bigo}[1]{\ensuremath{O \left( #1 \right)}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Domain adaptation experiments
\newcommand{\amazon}{{\bf A}}
\newcommand{\dslr}{{\bf D}}
\newcommand{\webcam}{{\bf W}}
\newcommand{\svhn}{{\bf SVHN}}
\newcommand{\mnist}{{\bf MNIST}}
\newcommand{\mm}{{\bf MM}}
\newcommand{\textrightarrow}{\ensuremath{\to}}


% kilian
\newcommand{\eat}[1]{} 

==> fastEnsemble - arXiv/method.tex <==
%!TEX root=main.tex
\section{Snapshot Ensembling}
\label{sec:method}



%\begin{table}[]
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|l|c|c||c|c|}
%\hline
%  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%Method    & Single model performance & Diversity  & Efficiency   & Ensemble performance \\ \hline
%Ensemble independent fully converged models & high & high & low  & high   \\ \hline
%Ensemble independent premature models       & low & high  & high & low   \\ \hline
%Ensemble models at different epochs         & high & low & high & low   \\ \hline
%Implicit ensemble (e.g., Dropout)           & high & low & high &    \\ \hline
%%   &  & % &  \\
%%   &  &  &  \\
%\hline
%\end{tabular}
%}
%
%\caption{Different ways of ensembling neural networks}
%\label{my-label}
%\end{table}

% \subsection{Learn free ensembles}
Snapshot Ensembling produces an ensemble of accurate and diverse models from a single training process. At the heart of Snapshot Ensembling is an optimization process which visits several local minima before converging to a final solution. We take model snapshots at these various minima, and average their predictions at test time.

Ensembles work best if the individual models (1) have low test error and (2) do not overlap in the set of examples they misclassify.
Along most of the optimization path, the weight assignments of a neural network tend not to correspond to low test error.
In fact, it is commonly observed that the validation error drops significantly only after the learning rate has been reduced, which is typically done after several hundred epochs.
Our approach is inspired by the observation that training neural networks for fewer epochs and dropping the learning rate earlier has minor impact on the final test error~\citep{loshchilov2016sgdr}.
This seems to suggest that local minima along the optimization path become promising (in terms of generalization error) after only a few epochs.

%To form a meaningful ensemble, each snapshot model should produce as few errors as possible. However, the set of errors that are made by any given snapshots should be disjoint from that of other snapshots to reduce the variance of the ensemble.
%Therefore, it is ideal to take snapshots in the local minimum where the model achieves acceptable accuracy. During a typical training process, the optimization trajectory leads the model to only one such local minimum. SGD optimization in high dimensional spaces tends to converge to high-error saddle points when the learning rate is large \citep{dauphin2014identifying}. These saddle points can be escaped by dropping the learning rate to a low value, which attracts the model to a better local minimum. Since typical learning rate schedules lower the learning rate only once, only the final converged solution will be an accurate local minimum.

%In order to discover multiple viable solutions, we perturb the model after it has converged to a local minimum. By raising the learning rate, the model escapes the local minimum and can therefore converge to alternate solutions when the learning rate is lowered again. Repeating this process creates an optimization trajectory which visits multiple low-error solutions, each of which produces different predictions on test data. By taking a model ``snapshot'' at each of these solutions, we obtain several accurate models which are prime for ensembling.



% \begin{wrapfigure}{r}{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.25\textwidth]{figures/lr_schedule-crop.pdf}
%     \caption{bla}
%     \label{fig:cosine}
% \end{wrapfigure}
\begin{wrapfigure}{r}{0.5\textwidth}
    \includegraphics[width=0.5\textwidth]{figures/train_loss.pdf}
    \caption{\small Training loss of 100-layer DenseNet on CIFAR10 using standard learning rate (blue) and $M=6$ cosine annealing cycles (red). The intermediate models, denoted by the dotted lines, form an ensemble at the end of training.}
    \label{fig:loss_curve}
\end{wrapfigure}
\para{Cyclic Cosine Annealing.}
To converge to multiple local minima, we follow a cyclic annealing schedule as proposed by~\citet{loshchilov2016sgdr}.
We  lower the learning rate at a very fast pace, encouraging the model to converge towards its first local minimum after as few as $50$ epochs. The optimization is then continued at a larger learning rate, which perturbs the model and dislodges it from the minimum. We repeat this process several times to obtain multiple convergences.
Formally, the learning rate $\alpha$ has the form:
%
\begin{equation}
\label{eq:lr-cycle}
\alpha(t) = f \left(\text{mod}\left(t-1,\left\lceil T/M \right\rceil\right)\right),
\end{equation}
%
where $t$ is the iteration number, $T$ is the total number of training iterations, and $f$ is a monotonically decreasing function.
In other words, we split the training process into $M$ cycles, each of which starts with a large learning rate, which is annealed to a smaller learning rate. The large learning rate $\alpha=f(0)$ provides the model enough energy to escape from a critical point, while the small learning rate $\alpha=f(\lceil T/M \rceil)$ drives the model to a well behaved local minimum. In our experiments, we set $f$ to be the shifted cosine function proposed by \cite{loshchilov2016sgdr}:
\begin{equation}
\label{eq:lr-cosine}
\alpha(t) = \frac{\alpha_0}{2}\left(\cos\left(\frac{\pi\text{mod}(t-1,\lceil T/M\rceil)}{\lceil T/M\rceil}\right)+1\right),
\end{equation}
%
where $\alpha_0$ is the initial learning rate.
Intuitively, this function anneals the learning rate from its initial value $\alpha_0$ to $f(\lceil T/M \rceil) \approx 0$ over the course of a cycle. Following \citep{loshchilov2016sgdr}, we update the learning rate at each iteration rather than at every epoch. This improves the convergence of short cycles, even when a large initial learning rate is used.

% Note that this strategy was also used by \cite{loshchilov2016sgdr} and \cite{leslie2016cyclical} recently. However, their aim is to obtain a best single model at the end of training, and this difference will lead to different considerations in designing the learning rate cycles. In particular, as our aim is to obtain strong neural network ensembles, instead of just pursuing an accurate model at the end of training, larger initial learning rate is usually preferred. This helps to speed up the training for the first few blocks, and tends to push the models converging to more diversified critical points. Although larger initial learning rate may degrade the performances of each single model, it benefits the final ensemble.


% We introduce a simple method to obtain multiple neural networks for effective model ensembling in one single training process, with the same amount of computational cost as training a single model in a usual way, but with significantly improved performance. Our basic idea is to collect models at different points along the training path for ensembling. However, traditional way of training neural networks has the learning rate gradually decaying from a larger value to some smaller value, which makes ensembling models from different iterations ineffective, because earlier models correspond to large learning rate are not accurate enough, while later models correspond to small learning rate strongly correlate with each other. As a consequence, naively ensembling models at different points of the training process does not lead to any improvement in practice.

% To collect intermediate neural networks in a single training pass to form meaningful ensembles, it is important to have the model occasionally converge into a local minimum or saddle points, where the model achieves acceptable accuracy. In fact, \cite{dauphin2014identifying} show that the saddle points are prevalent in high dimensional spaces, and many of them give relatively low training loss. Therefore, we can take a ``snapshot'' for the temporarily converged model for later ensembling. We then need to endow the model enough energy to escape from these local minima or saddle points again to search for better ones. By repeating this process, we can take many ``snapshots'' of models along the path while searching for optimal weights. These models yields good accuracy as they all settled in critical points, and they tend to produce different predictions on test data as the critical points are different in high dimensional space. Therefore, effective ensemble can be ensured.

% Specifically, we split the training process into $K$ stages, each of which has a full learning rate annealing cycle, i.e., we have the learning rate starting from a large value and gradually decreasing to a small value. The large learning rate in each stage gives the model enough energy to escape from a critical point, and the small learning rate will drive the model to a well behaved local minimum or saddle points. Formally, the learning rate $\alpha$ in our method has the form:





% \para{Learning rate annealing.}
% The learning rate function $f$ can take many forms of monotonically decreasing function. Some popular choices are multi-step functions, linear/exponential decay functions and the shifted cosine function recently used by \cite{loshchilov2016sgdr}. The cosine function is relatively easy to use, as we only need to specify a maximum learning rate, which is usually set to the initial learning rate; and a minimum learning rate, which is usually set to 0. Thus we adopt the cosine shape learning rate in our experiments. However, instead of updating the learning rate at each epoch as in \cite{loshchilov2016sgdr}, we have the learning rate updated at each iteration, so as to produce a more smooth annealing curve. This is important because in our case each block has fewer epochs, and changing learning rate at each epoch tend to give less converged models, especially when the initial learning rate is large. Specifically, the learning rate annealing function used in our experiment is
% \begin{equation}
% \label{eq:lr-cosine}
% \alpha(t) = \frac{\alpha_0}{2}\left(\cos\left(\frac{\pi\text{mod}(t-1,T/K)}{T/K}\right)+1\right),
% \end{equation}
% where $\alpha_0$ is the initial learning rate.


%The obtained model ensemble achieves significant improved performance over the single model trained using conventional learning rate scheduling, without adding further training cost overhead. In other words, the model ensemble is obtained for free or at relatively low cost.

% \para{Number of learning rate annealing cycles.}
% Empirically, we find that the algorithm is robust to the number of cycles of annealing learning rate. In practice, splitting the entire training process into 3 to 10 cycles works well.


\para{Snapshot Ensembling.}
\autoref{fig:loss_curve} depicts the training process using cyclic and traditional learning rate schedules. At the end of each training cycle, it  is apparent that the model reaches a local minimum with respect to the training loss. Thus, before raising the learning rate, we take a ``snapshot'' of the model weights (indicated as vertical dashed black lines). After training $M$ cycles, we have $M$ model snapshots, $f_1 \ldots f_M$, each of which will be used in the final ensemble. It is important to highlight that the total training time of the $M$ snapshots is the same as training a model with a standard schedule (indicated in blue). In some cases, the standard learning rate schedule achieves lower training loss than the cyclic schedule; however, as we will show in the next section, the benefits of ensembling outweigh this difference.

\para{Ensembling at Test Time.}
The ensemble prediction at test time is the average of the last $m$ ($m \leq M$) model's softmax outputs. Let $\mathbf{x}$ be a test sample and let $h_i \left( \mathbf{x} \right)$ be the softmax score of snapshot $i$. The output of the ensemble is a simple average of the last $m$ models:
%
$
  h_{\text{Ensemble}} = \frac{1}{m} \sum_{0}^{m-1} h_{M-i} \left( \mathbf{x} \right).
  % \label{eq:ensemble}
$
%
We always ensemble the last $m$ models, as these models tend to have the lowest test error.



% In some scenarios, one may have a pretrained model, and would like to have more models to form an ensemble. The easiest way is to retrain models from scratch, which however can be computationally expensive. In fact, to obtain model ensemble more efficiently, one can first disturb the pretrained model, and retain the model to converge. Although there are many ways to disturb the model, we propose to use large learning rate to push the weights away from the current position, and then anneal the learning rate to make the weights converges to a different point.


% \subsection{Further increasing the model diversity and reducing computational cost}
% \para{Subsample the training set.}
% During each learning rate cycle, we can subsample a subset of the training set as in the \emph{bagging} method. Since each model is trained on a different subset of training data, the diversity will increase, and the number of iterations to update the model can be lowered.

% \para{Subsample the model.}
% We can also subsample the model at a previous cycle and retrain this model, so as to further lower the correlation between models. Model subsampling may also reduce the training cost as the model size shrinks.


%\subsection{Reducing evaluation cost}
%
%\para{Ensemble the last few models.}
% In the free ensemble method, one can always start with the model from the end of the last block. When test time budget allows, we can add an additional model to the ensemble from the last iteration of the previous stage.
%
%\para{Model distillation.}
% Using the model distillation method~\citep{hinton2015distilling}, we can transfer the knowledge of the model ensemble into a single mode. The student network can be initialized with the model from the last iteration, and it would only require very few iterations to update the model.










==> fastEnsemble - arXiv/related_work.tex <==
%!TEX root=main.tex
\section{Related Work}

Neural network ensembles have been widely studied and applied in machine learning \citep{hansen1990neural,krogh1995neural}. However, most of these prior studies focus on improving the generalization performance, while few of them address the cost of training ensembles.
%This may be explained by the fact that one decade ago both the size of datasets and models were relatively small, and it was affordable to train tens or even hundreds of networks for model averaging. But the situation is changing rapidly. On one hand, many of the datasets we have now contain millions of samples; On the other hand, researchers have to train very deep networks to achieve good performances on these large scale datasets. Even with the modern GPUs, a deep network may take days or weeks to train. Under limited resources, it becomes important to address the problem of high training cost of neural network ensembles. Several recent works focus on reducing the test time cost of ensembles, by transferring or distilling the ``knowledge" of cumbersome ensembles into smaller networks \citep{bucilu¨£2006model,hinton2015distilling}.

%\gp{It might be good to start off with something like: The most commonly used approach for ensembling classification models is averaging the softmax outputs of several models. While simple, it is highly effective for neural networks and is one of the most common ensembling methods used today.}

As an alternative to traditional ensembles, so-called ``implicit'' ensembles have high efficiency during both training and testing \citep{dropout,wan2013regularization,stochastic,singh2016swapout,krueger2016zoneout}.
The Dropout \citep{dropout} technique creates an ensemble out of a single model by ``dropping'' --- or zeroing --- random sets of hidden nodes during each mini-batch. At test time, no nodes are dropped, and each node is scaled by the probability of surviving during training.
\citeauthor{dropout} claim that Dropout reduces overfitting by preventing the co-adaptation of nodes.
An alternative explanation is that this mechanism creates an exponential number of networks with shared weights during training, which are then implicitly ensembled at test time.
DropConnect \citep{wan2013regularization} uses a similar trick to create ensembles at test time by dropping connections (weights) during training instead of nodes.
The recently proposed Stochastic Depth technique \citep{stochastic} randomly drops layers during training to create an implicit ensemble of networks with varying depth at test time.
% Stochastic Depth has a strong regularization effect and tends to outperform Dropout on very deep networks \citep{stochastic}. 
Finally, Swapout \citep{singh2016swapout} is a stochastic training method that generalizes Dropout and Stochastic Depth. From the perspective of model ensembling, Swapout creates diversified network structures for model averaging. Our proposed method similarly trains only a single model; however, the resulting ensemble is ``explicit'' in that the models do not share weights.  Furthermore, our method can be used in conjunction with any of these implicit ensembling techniques.

Several recent publications focus on reducing the \emph{test time cost} of ensembles, by transferring the ``knowledge" of cumbersome ensembles into a single model \citep{bucilu2006model,hinton2015distilling}. \citet{hinton2015distilling} propose to use an ensemble of multiple networks as the target of a single (smaller) network.
% In order to effectively train the new network, a high temperature is used to soften the probability distribution over classes. 
Our proposed method is complementary to these works as we aim to reduce the \emph{training} cost of ensembles rather than the test-time cost.

%There are several recently proposed training mechanisms to improve the power of explicit ensembles.
%\citet{laine2016temporal} propose a temporal ensembling method for semi-supervised learning, which achieves consensus among models trained with different regularization and augmentation conditions.
%%This method has been shown to outperform the model at the most recent training epoch.
%Recently, \cite{moghimiboosted} show that boosting can be applied to convolutional neural networks to create strong ensembles.

Perhaps most similar to our work is that of \citet{swann1998fast} and \citet{xie2013horizontal}, who explore creating ensembles from slices of the learning trajectory.
\citeauthor{xie2013horizontal} introduce the \emph{horizontal and vertical} ensembling method, which combines the output of networks within a range of training epochs.
More recently, \citet{jean2014using} and \citet{sennrich2016edinburgh} show improvement by ensembling the intermediate stages of model training. \citet{laine2016temporal} propose a temporal ensembling method for semi-supervised learning, which achieves consensus among models trained with different regularization and augmentation conditions for better generalization performance. Finally, \cite{moghimiboosted} show that boosting can be applied to convolutional neural networks to create strong ensembles.
Our work differs from these prior works in that we force the model to visit multiple local minima, and we take snapshots \emph{only} when the model reaches a minimum. We believe this key insight allows us to leverage more power from our ensembles.

Our work is inspired by the recent findings of \cite{loshchilov2016sgdr} and \cite{leslie2016cyclical}, who show that cyclic learning rates can be effective for training convolutional neural networks. The authors show that each cycle produces models which are (almost) competitive to those learned with traditional learning rate schedules while requiring a fraction of training iterations. Although model performance temporarily suffers when the learning rate cycle is restarted, the performance eventually surpasses the previous cycle after annealing the learning rate. The authors suggest that cycling perturbs the parameters of a converged model, which allows the model to find a better local minimum.
%Thus this method can generate several accurate and diverse models throughout the training process rather than producing a single model at the end of training.
We build upon these recent findings by (1) showing that there is significant diversity in the local minima visited during each cycle and (2) exploiting this diversity using ensembles. We are not concerned with speeding up or improving the  training of a single model; rather, our goal is to extract an ensemble of classifiers while following the optimization path of the final model.






==> fastEnsemble - arXiv/result/caption.tex <==
%!TEX root=../main.tex
\newcommand{\resultcaption}{Error rates (\%) on CIFAR and SVHN datasets. $L$ denotes the network depth and $k$ its \stepsizename{}. Results that surpasses all competing methods are {\textbf{bold}} and the overall best results are {\color{blue}\textbf{blue}}. ``+'' indicates standard data augmentation (translation and/or mirroring). $\ast$ indicates results run by ourselves. All the results of \methodnameshort{} without data augmentation (C10, C100, SVHN) are obtained using Dropout. \methodnameshort{}s achieve lower error rates while using fewer parameters than ResNet. 
Without data augmentation, \methodnameshort{} performs better by a large margin.
}


==> fastEnsemble - arXiv/result/table.tex <==
\setlength\tabcolsep{2pt}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|c}
\hline
\multicolumn{1}{c|}{Method} & \multicolumn{1}{l}{Depth} & \multicolumn{1}{l|}{Params} & C10 & C10+ & C100 & C100+ & SVHN \\ \hline
Network in Network \citep{netinnet} & - & - & 10.41 & 8.81 & 35.68 & - & 2.35 \\
All-CNN \citep{allcnn} & - & - & 9.08 & 7.25 & - & 33.71 & - \\
Deeply Supervised Net \citep{dsn} & - & - & 9.69 & 7.97 & - & 34.57 & 1.92 \\
Highway Network \citep{highway} & - & - & - & 7.72 & - & 32.39 & - \\ \hline
FractalNet \citep{fractalnet} & 21 & 38.6M & 10.18 & 5.22 & 35.34 & 23.30 & 2.01 \\
with Dropout/Drop-path & 21 & 38.6M & 7.33 & 4.60 & 28.20 & 23.73 & 1.87 \\ \hline
ResNet \citep{resnet} & 110 & 1.7M & - & 6.61 & - & - & - \\ \hline
ResNet (reported by \citet{stochastic}) & 110 & 1.7M & 13.63 & 6.41 & 44.74 & 27.22 & 2.01 \\ \hline
ResNet with Stochastic Depth \citep{stochastic} & 110 & 1.7M & 11.66 & 5.23 & 37.80 & 24.58 & 1.75 \\
 & 1202 & 10.2M & - & 4.91 & - & - & - \\ \hline
Wide ResNet \citep{wide} & 16 & 11.0M & - & 4.81 & - & 22.07 & - \\
 & 28 & 36.5M & - & 4.17 & - & 20.50 & - \\
with Dropout & 16 & 2.7M & - & - & - & - & 1.64 \\ \hline
ResNet (pre-activation) \citep{identity-mappings} & 164 & 1.7M & 11.26$^\ast$ & 5.46 & 35.58$^\ast$ & 24.33 & - \\
\multicolumn{1}{c|}{} & 1001 & 10.2M & 10.56$^\ast$ & 4.62 & 33.47$^\ast$ & 22.71 & - \\ \hline
\methodnameshort{} $(L=40, k=12)$ & 40 & 1.0M & \textbf{7.00} & 5.24 & \textbf{27.55} & 24.42 & 1.79 \\
\methodnameshort{} $(L=100, k=12)$ & 100 & 7.0M & {\color{blue}\textbf{5.77}} & \textbf{4.10} & \textbf{23.79} & \textbf{20.20} & 1.67 \\
\methodnameshort{} $(L=100, k=24)$ & 100 & 27.2M & \textbf{5.83} & {\color{blue}\textbf{3.74}} & {\color{blue}\textbf{23.42}} & {\color{blue}\textbf{19.25}} & {\color{blue}\textbf{1.59}} \\ \hline
\end{tabular}%
}
\caption{\resultcaption}
\label{my-label}
\end{table} 

==> introOLD.tex <==
Averaging classifiers is an effective method to reduce model variance by approximating the expected classifier. Ensemble methods~\citep{breiman2001random,caruana2004ensemble,hansen1990neural,krogh1995neural,zhou2002ensembling} leverage this fact to obtain improved generalization performance~\cite{koren2009bellkor}. 
For example, the Random Forests~\cite{breiman2001random}  algorithm elevates the modest CART~\cite{breiman1984classification} algorithm to one of the most competitive classifiers within machine learning. 
Here, slightly modified CART trees are bagged~\cite{breiman2001random}, where each tree is trained on a different subset of the data (drawn uniformly with replacement) and splits are randomized. The additional randomization of the decision trees leads to high variance classifiers. This is advantageous as the ensemble size can be very large (in practice often exceeding 10,000 CART trees) due to the extremely efficient ID3 algorithm~\cite{quinlan1986induction}. The large number of classifiers ensures that even in the presence of high variance the ensemble average approaches the expected model (which would have zero model variance).  

In the wake of deep learning, ensembling is just as important as it has ever been. Nowadays most high profile competitions (e.g. Imagenet~\cite{deng2009imagenet} or Kaggle\footnote{\url{www.kaggle.com}}) are won by ensembles of deep learning architectures. As neural networks are often initialized with random weights, there appears to be a sufficient amount of natural variation that allows all networks to be trained on the entire data set. 

Training deep networks is computationally expensive and can last for days or even weeks even on high performance hardware with GPU acceleration. Training ensembles of them increases the cost linearly and quickly becomes prohibitive for most researchers without access to industrial scale computational resources. Although the training of deep net ensembles can be trivially parallelized, few have access to sufficient GPU servers that can be deployed in parallel for long durations. As a result, ensembles of deep nets are typically small---averaging only a hand-full of classifiers. Consequently, the ensemble average still has high variance and does not approach the expected model. 

% The ensemble method is very effective for neural networks. In most cases, neural network ensembles yield significantly better generalization performance than a single network.
% The recent winners of the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) \citep{imagenet} have all used multiple networks for their final predictions \citep{szegedy2015going,smallfilter,resnet}.
% Researchers have found that independently trained neural networks tend to make different mistakes on test data, and thus averaging the softmax scores or using a majority voting scheme can greatly reduce the chance of a wrong prediction. The diversity amongst models is a product of random initialization and training with stochastic gradient descent (SGD), coupled with the high degree of nonlinearity in neural networks \gp{Should this mention non-convexity?}. Due to its simpleness and effectiveness, the ensemble method is widely used in deep learning applications.

% Although neural networks ensembles have been widely studied and utilized \citep{hansen1990neural,krogh1995neural}, most existing works focuses on improving the generalization performance, with little concern about the cost of training ensembles. This may be explained by the fact that, until recently, the sizes of both datasets and models were relatively small, making it affordable to train tens or even hundreds of networks for model averaging. However, the situation is rapidly changing. Many datasets now contain millions of samples, and researchers must train very deep networks to achieve good performance on these large scale datasets. Even with the modern GPUs, a deep network may take days or weeks to train. Under limited resources, it becomes important to address the large cost of training neural network ensembles. 

One useful feature of SGD is that SGD does not get caught in local minima that it happens upon during the training process.
In fact, SGD can even escape the attraction of a local minimum.
Somehow cite Bengio.
Therefore, rather than preventing a model from visiting local minima, we allow the model to visit many local minima over the course of optimization, knowing that we can escape it again.
We take a model snapshot when we converge to a local minimum, and then perturb the model to let it escape that local minimum. Therefore, we end up with several models that have converged to various minima, which give us enough variety to converge to several different models.

% There are several methods which can lower this cost to a certain extent. 
% For example, one can use shorter networks for model averaging, or train each network for fewer iterations.
% While these methods reduce training time, both may sacrifice accuracy on a sufficiently challenging dataset.
% Even with careful hyperparameter selection, such an ensemble might 
% not outperform the simple baseline: training a single network under the same amount of cost.
% Alternatively, one could train a single deep network, but ensemble intermediate models at different iterations of training.
% This method does not introduce any additional training
% beyond training a single model, yet the accuracy gain is often insignificant as there is little diversity amongst the different
% training iterations.


%Although neural networks ensembles have been widely studied and applied in machine learning \citep{hansen1990neural,krogh1995neural}, most of existing works focus on improving the generalization performance, while few of them address the cost of training ensembles. This may be explained by the fact that one decade ago both the size of datasets and models were relatively small, and it was affordable to train tens or even hundreds of networks for model averaging. But the situation is changing rapidly. On one hand, many of the datasets we have now contain millions of samples; On the other hand, researchers have to train very deep networks to achieve good performances on these large scale datasets.
%
%Even with the modern GPUs, a deep network may take days or weeks to train. Under limited resources, it becomes important to address the problem of high training cost of neural network ensembles. Several recent works focus on reducing the test time cost of ensembles, by transferring or distilling the ``knowledge" of cumbersome ensembles into smaller networks \citep{bucilu¨£2006model,hinton2015distilling}.
%

% In recent years, researchers have developed effective techniques which create ``implicit'' ensembles from single networks \citep{dropout,wan2013regularization,stochastic,singh2016swapout,krueger2016zoneout}. For example, the Dropout \citep{dropout} method randomly drops nodes in the hidden layers during each mini-batch of training. This can be viewed as training exponential number of networks with heavy parameter sharing. At test time, these models are averaged to make the final prediction. The recently proposed stochastic depth network \citep{stochastic} and Swapout \citep{singh2016swapout} algorithm create similar implicit ensembles at test time. \gp{Maybe worth mentioning the ``Resnets are ensembles\ldots'' paper?}

In this paper, we introduce a simple idea to obtain a cheep yet effective neural network ensembles under a limited training budget.
Our method produces multiple neural networks that achieve a remarkable balance between diversity and accuracy, yet only requires the \emph{same cost training a single network}. We draw inspiration from the recent finding of \cite{loshchilov2016sgdr} and \cite{leslie2016cyclical} that cyclical learning rates give significant improvement over commonly used learning rate scheduling. Cyclical learning rates split the training process into multiple blocks, each of which has a full learning rate annealing cycle. In each block, large learning rates perturbs a well converged model and small learning rates quickly drive the model towards convergence at a new minimum. Consequently, each block (or learning rate cycle) provides a candidate model for ensembling. This disturbance at the beginning of each block produces intermediate models with substantial diversity, and are therefore far more effective for ensembling than intermediate models from a conventional learning rate schedule. 

The proposed method has several remarkable advantages: 1) it is possible to retrieve models with good performance early in the training process, as noted by \citet{loshchilov2016sgdr}; 2) it always gives a complete single model at the end of training, and one can further improve its performance by simply ensembling more models provided test time budget allows;
%, making it useful for test time cost sensitive learning; 
3) the method is general and is compatible with many other effective tools in deep learning, such as Bagging, Boosting, Dropout, Swapout, Stochastic depth and the Dense-sparse-dense training flow. In fact, our method can be even more effective when combined with some of these other techniques.

We show on several popular benchmark datasets that our method yields state-of-the-art performance with the ResNet~\citep{identity-mappings} and DenseNet~\citep{huang2016densely} architecture under the same amount of training cost as in previous works. We also introduce how to further improve model diversity and reduce cost at training time.

%Tested on ResNet and DenseNet. Also introduces how to reducing test time computation.









==> result/caption.tex <==
%!TEX root=../main.tex
\newcommand{\resultcaption}{Error rates (\%) on CIFAR and SVHN datasets. $L$ denotes the network depth and $k$ its \stepsizename{}. Results that surpasses all competing methods are {\textbf{bold}} and the overall best results are {\color{blue}\textbf{blue}}. ``+'' indicates standard data augmentation (translation and/or mirroring). $\ast$ indicates results run by ourselves. All the results of \methodnameshort{} without data augmentation (C10, C100, SVHN) are obtained using Dropout. \methodnameshort{}s achieve lower error rates while using fewer parameters than ResNet. 
Without data augmentation, \methodnameshort{} performs better by a large margin.
}


==> result/table.tex <==
\setlength\tabcolsep{2pt}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|c}
\hline
\multicolumn{1}{c|}{Method} & \multicolumn{1}{l}{Depth} & \multicolumn{1}{l|}{Params} & C10 & C10+ & C100 & C100+ & SVHN \\ \hline
Network in Network \citep{netinnet} & - & - & 10.41 & 8.81 & 35.68 & - & 2.35 \\
All-CNN \citep{allcnn} & - & - & 9.08 & 7.25 & - & 33.71 & - \\
Deeply Supervised Net \citep{dsn} & - & - & 9.69 & 7.97 & - & 34.57 & 1.92 \\
Highway Network \citep{highway} & - & - & - & 7.72 & - & 32.39 & - \\ \hline
FractalNet \citep{fractalnet} & 21 & 38.6M & 10.18 & 5.22 & 35.34 & 23.30 & 2.01 \\
with Dropout/Drop-path & 21 & 38.6M & 7.33 & 4.60 & 28.20 & 23.73 & 1.87 \\ \hline
ResNet \citep{resnet} & 110 & 1.7M & - & 6.61 & - & - & - \\ \hline
ResNet (reported by \citet{stochastic}) & 110 & 1.7M & 13.63 & 6.41 & 44.74 & 27.22 & 2.01 \\ \hline
ResNet with Stochastic Depth \citep{stochastic} & 110 & 1.7M & 11.66 & 5.23 & 37.80 & 24.58 & 1.75 \\
 & 1202 & 10.2M & - & 4.91 & - & - & - \\ \hline
Wide ResNet \citep{wide} & 16 & 11.0M & - & 4.81 & - & 22.07 & - \\
 & 28 & 36.5M & - & 4.17 & - & 20.50 & - \\
with Dropout & 16 & 2.7M & - & - & - & - & 1.64 \\ \hline
ResNet (pre-activation) \citep{identity-mappings} & 164 & 1.7M & 11.26$^\ast$ & 5.46 & 35.58$^\ast$ & 24.33 & - \\
\multicolumn{1}{c|}{} & 1001 & 10.2M & 10.56$^\ast$ & 4.62 & 33.47$^\ast$ & 22.71 & - \\ \hline
\methodnameshort{} $(L=40, k=12)$ & 40 & 1.0M & \textbf{7.00} & 5.24 & \textbf{27.55} & 24.42 & 1.79 \\
\methodnameshort{} $(L=100, k=12)$ & 100 & 7.0M & {\color{blue}\textbf{5.77}} & \textbf{4.10} & \textbf{23.79} & \textbf{20.20} & 1.67 \\
\methodnameshort{} $(L=100, k=24)$ & 100 & 27.2M & \textbf{5.83} & {\color{blue}\textbf{3.74}} & {\color{blue}\textbf{23.42}} & {\color{blue}\textbf{19.25}} & {\color{blue}\textbf{1.59}} \\ \hline
\end{tabular}%
}
\caption{\resultcaption}
\label{my-label}
\end{table} 
